Text Recognition -- Real World Data and Where to Find Them

We present a method for exploiting weakly annotated images to improve text extraction pipelines. The approach uses an arbitrary end-to-end text recognition system to obtain text region proposals and their, possibly erroneous, transcriptions. The proposed method includes matching of imprecise transcription to weak annotations and edit distance guided neighbourhood search. It produces nearly error-free, localised instances of scene text, which we treat as "pseudo ground truth" (PGT). We apply the method to two weakly-annotated datasets. Training with the extracted PGT consistently improves the accuracy of a state of the art recognition model, by 3.7~\% on average, across different benchmark datasets (image domains) and 24.5~\% on one of the weakly annotated datasets.

==> reviews.tex <==
\clearpage


\section{Rebuttal}

We thank the reviewers for the comments. In the following, we address them, copied verbatim.
% We believe the readability has increased greatly, hopefully clarifying the doubts.

\noindent\rule{\columnwidth}{0.5pt}

\textcolor{Blue}{[R1, C1] The description in the paper should be improved, such
as the meanings of the “?” in TABLE II(PP 6) , and
“zeros.u” in the last line of page 5, etc. }

These were typos/incorrect references which have been fixed, as well as any other we have found.

\textcolor{Blue}{[R1, C2] Experiments (TABLE V) have been conducted on some
datasets, but the results are less advanced than the SOTA
methods, the authors should make more analysis on the
experimental results.}

We added the second-best SOTA performance to Table \ref{tab:strb-alphanum}. This shows that our model achieves second-best performance on three different datasets. Furthermore, we have modified the conclusions to highlight that the adopted architecture is SOTA among those with public code-base.

Current SOTA on most datasets is \cite{litman2020scatter}, which is a CVPR 2020 publication and achieves the top results with different model configurations on different datasets.

We propose a new approach for training text recognition via weakly-supervised training. The method is not architecture-specific, improvements in training data are orthogonal to improvements in model architecture and there is no reason to believe the method would not work with future SOTA architectures.

\textcolor{Blue}{[R1, C3] The size of the data UTi in TBALE II should be given,
as well as that of the ABCi dataset.}

The size of each of these datasets was reported in Table I (UT) and Table III (ABC), now Figure \ref{fig:pgt_numbers} and Table \ref{tab:mining}.

We believe there may have been some confusion due to the heading ``Training dataset - example \%'' in Table II, which refers to dataset example \% per each batch. We have clarified this.

\textcolor{Blue}{[R1, C4] The proposed method is related to pseudo-labelling
techniques, and some comparative experiments are necessary.}

We have included experiments of pseudo-labelling \cite{lee2013pseudo} with confidence tresholding, as done by previous researches. The best model's performance is compared to the proposed method and fully-supervised one in Figure \ref{fig:ut_acc} and more detailed results, as well as description of the approach, in Appendix \ref{app:semi-sup}.

\textcolor{Blue}{[R1, C5] As the description in Page 6, “we split large (about
4K) images into 16 blocks ensuring no text instance is
split and discard those with no text”. In my opinion, this
is not reasonable. }

It is just a technicality used during the PGT generation process and the results should not differ from running the whole image at once on a bigger GPU - splitting images that are too big is a common practice. For text detection/recognition, other options such as re-scaling are not reasonable as small texts may get lost. 

\noindent\rule{\columnwidth}{0.5pt}

\textcolor{Blue}{[R2, C1] The experimental results of "number of boxes with text
generated" in Table I and Table III cannot prove the
effectiveness of the proposed PGT method, as no direct
quantitative results for the accuracy of PGT are presented.}

We added an analysis of the errors/ambiguities of the PGT on both datasets, see Subsection\ref{subsec:pgt_acc} and Appendix \ref{app_pgt_acc}.

We would like to point out that while the accuracy is interesting to know, high accuracy does not imply better model - very simple synthetic data may have 100 \% accuracy, yet little additional value when training recognition models. Figure \ref{fig:ut_acc} and Tables \ref{tab:uber-test} and \ref{tab:strb-all} show the effectiveness in terms of improvements to the baseline model (no architecture changes, only the PGT data has been added).

\textcolor{Blue}{[R2, C2] It seems that the application of the proposed method is
limited as other large scale weakly annotated databases may
not be available. And different databases may have
different format of annotations.}

We added more examples of weakly annotated databases in Figure \ref{fig:weak_sources}.

Of course, there is the issue of availability in terms of data usage policies but this changes dynamically - data that were allowed for use in research are not available anymore and vice-versa.

The different format of annotations is not a problem as long as it is textual data that may appear in the image and there are many such databases. The PGT-GEN methods handles texts at different granularities, be it separate words or some longer phrases. Converting from different formats (JSON, XML, ...) is just a technicality that can be solved easily.

\textcolor{Blue}{[R2, C3] On page 3, an example of annotation text is given,
"Sherlock Holmes, consulting detective", however, the
phrase "consulting detective" is not found in the given A
and G. }

This was a mistake - now fixed.

\noindent\rule{\columnwidth}{0.5pt}
% \textcolor{Blue}{[R3, C1] The proposed PGT is not an intelligent method, but
% includes lots of rules with many threshholds. Meanwhile, it
% is not hard to find the idea for text recognition.}

% TODO

\textcolor{Blue}{[R3, C2] The paper is wirtten almost full of text. There is few
figures to show the framework of the proposed method.
Meanwhile, it it better to introduce the operations of the
proposed method with pseudo codes.}

We have rewritten Section \ref{sec:pgt_gen} (PGT generation) entirely - introduced Algorithm \ref{alg_pgt} and changed the formalization. We have also visualized the training with PGT procedure in Figure \ref{fig:pgt_training} and changed Tables I and III in the original paper to a plot in Figure \ref{fig:pgt_numbers} and Table III to Figure \ref{fig:ut_acc}. The original tables can still be found in Appendix \ref{app:add_exps}. Some less important parts were moved to Supplementary material. We believe the changes have increased the readability greatly.

\textcolor{Blue}{[R3, C3] The recognition accuracy with the proposed method is not
obviously better than state-of-the-art recognition methods. }

Already addressed in [R1, C2]



==> tables/amazon-mining.tex <==

\begin{table}

	\centering


	\begin{tabular}{c|r|r|r}
% 		\hline
		Iteration / Mined: & with neigh. s. & w/o neigh. s. & $\Delta $ \\
		\hline
		 1 & 1,536,583 & 1,234,219 & 302,364 \\
% 		\hline
		 2 & 1,581,109 & 1,354,219 & 226,890 \\
% 		 \hline
		 3 & 1,594,333 & 1,375,571 & 218,762 \\
		\hline
		
	\end{tabular} 

\vspace{-1ex}
	\caption{Pseudo-ground truth (PGT) generation performance on the ABC dataset.
	The number of boxes  with text generated: 
	in total, without and with the neighbourhood search.}
	\label{tab:mining_amazon}
\end{table}

